PIMBALL: Binary Neural Networks in Spintronic Memory

Neural networks span a wide range of applications of industrial and commercial significance. Binary neural networks (BNN) are particularly effective in trading accuracy for performance, energy efficiency or hardware/software complexity. Here, we introduce a spintronic, re-configurable in-memory BNN accelerator, PIMBALL: Processing In Memory BNN AcceL(L)erator, which allows for massively parallel and energy efficient computation. PIMBALL is capable of being used as a standard spintronic memory (STT-MRAM) array and a computational substrate simultaneously. We evaluate PIMBALL using multiple image classifiers and a genomics kernel. Our simulation results show that PIMBALL is more energy efficient than alternative CPU, GPU, and FPGA based implementations while delivering higher throughput.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

==> mine/cramISCA19.tex <==
%\subsection{Computational RAM}
\noindent Without loss of generality,
%, we adapt
%In our work we use 
\arch\ uses  
Computational RAM (CRAM) as the spintronic PIM substrate~\cite{cram}.  The structure consists of an array of magnetic tunnel
junctions (MTJs) and can be used as a standard STT-MRAM memory array. Due to
desirable properties of MTJs, the memory is fast, low power, high density, and
non-volatile. Due to non-volatility, standby power is near zero. At the same time, MTJs are inherently compatible with logic operations. This
enables computation to take place {\em entirely} inside the memory array, without the
use of external logic or sense-amplifiers. This provides true PIM capability.
Further, the structure of the array allows for massively parallel computation.
%,
%which enables the computation to not only be energy efficient but capable of
%high throughput. 
%At the same time, we do not simply use the basic array structure
%from~\cite{cram}, but modify  

As we will detail in the following, however, the basic array structure from~\cite{cram} cannot support BNNs. 
Building upon this limited basic design~\cite{cram}, a key contribution
of our work is design space exploration for the memory cell architecture
(augmented with compute capability), which resulted in novel memory cell and array architectures enabling efficient BNNs in memory.

%We
%build upon this basic array structure from~\cite{cram} to enable efficient BNN processing,
%This resulted in novel memory cell and array
%architectures, as we will detail in the following. 
%Additionally, we use a cell design augmented with a Spin-hall effect (SHE) %channel similar to the one proposed in \cite{masoud2}.}

\vshrink{-.1}
\noindent{\bf Magnetic Tunnel Junction (MTJ):}
{The magnetic tunnel junction is the key
building block of the memory cells. MTJs
are resistive memory devices,
%they are 
characterized by 
%having 
two distinct resistance levels
%It is these two resistance levels which 
to represent logic 1 and logic 0.  Each MTJ has two magnetic layers, a fixed layer
and a free layer. The polarity of the free layer can change but the fixed
cannot. When the two layers are aligned, the MTJ is in the parallel (P) state,
which is considered to be logic 0. If the magnetic layers are not aligned, the
MTJ is in the anti-parallel (AP) state, which is considered to be logic 1. The
MTJ has a much higher resistance in the AP state than it does in the P state. 
The state can be changed by passing current through the MTJ, where the direction }
%of the
%current 
determines the final state. 

\vshrink{-.1}
%\subsubsection{CRAM Array}
\noindent{\bf Cell \& Array Architecture:}
{We consider three different configurations of the memory cells, which range from
1T1M (one transistor per MTJ or magnet) to 3T1M (three transistors per MTJ or magnet).}

\ignore{
As a baseline for comparison, we also adapt 2T1M (two transistors per magnet)
which is similar to the design in~\cite{cram}. 
%The
%base configuration is similar to previous CRAM designs. 
We also introduce {\em transposed} configurations of the array.
}
%

\ignore{
\begin{figure}[tp]
%\vshrink{.2}
\centering
\begin{subfigure}[t]{.45\columnwidth}
\centering
\includegraphics[scale=0.24]{Images/array/prev/cell.png}
\caption{2T1M }
\label{fig:2Tcell}
\end{subfigure}
%%%
\begin{subfigure}[t]{.45\columnwidth}
\centering
\includegraphics[scale=0.24]{Images/array/T/STT.png}
\caption{1T1M}
\label{fig:stt}
\end{subfigure}
\vshrink{.2}
\caption{Default 2T1M~\cite{cram} vs. 1T1M cell.}
%\label{fig:cell}
\vshrink{.6}
\end{figure}
}

%Two additional
%configurations are transposed versions of the CRAM array, described in Section
%\ref{sec:transpose}. 
Fig.\ref{fig:2Tcell} shows the default 2T1M cell architecture from~\cite{cram}, which
we include here as a baseline for comparison.
%used
%previously. 
%It is a 2T1M design, meaning each cell contains one MTJ and two
%access transistors. 
The array formed by these cells is identical to a standard 1T1M STT-MRAM array, except for an 
%addition of a few extra features. These include an 
additional access transistor per cell; the control signal {\em Logic Line}
(LL) which runs along the rows; and the control signal {\em Bit Line for Logic}
(BLL) which runs along the columns. 

%\vshrink{-.1}
%\noindent{\bf Operation Sematics (2T1M) \cite{cram}:}
\noindent{\bf Memory \& Logic Semantics (2T1M) \cite{cram}:}
If no computation is taking place, the array from Fig.\ref{fig:2Tcell} can serve exactly as an STT-MRAM array.
In this case, the WLM signal activates the access transistor $t_{M}$ (transistor for
memory), that connects MTJs to the bitline bar (BLB) on a per row basis. Cells
can then be read or written via the BL and BLB. The extra hardware enables
computation within the array. The second access transistor $t_{L}$
(transistor for logic), connects the MTJs to the LL. 
BLL controls this second transistor $t_{L}$.
When BLL is activated for multiple columns,
the MTJs 
in those columns, that are also in the same row, are connected together
via the shared LL. 
%

\begin{wrapfigure}{l}{0.3\textwidth}
\vshrink{.2}
%
\begin{minipage}{\linewidth}
\centering
%\captionsetup[subfigure]{justification=centering}
\captionsetup[subfigure]{justification=justified, width=\linewidth}
%   \includegraphics[scale=0.22]{Images/array/3T/cell_memory}
    \includegraphics[width=\linewidth]{Images/array/prev/cell.png}
    \subcaption{2T1M~\cite{cram}}
\label{fig:2Tcell}
\par\vfill
    \includegraphics[width=.85\linewidth]{Images/array/T/STT.png}
    \subcaption{1T1M}
\label{fig:stt}
\end{minipage}
%
\vshrink{.4}
%\caption{Default 2T1M vs. 1T1M cell.}
\caption{Cell architecture.}
\label{fig:basiccell}
\vshrink{.3}
\end{wrapfigure}

MTJs that are connected over LL in a row can act either as inputs or outputs of
a logic gate. Hence, the result of the logic gate directly changes the state of the MTJ designated as the output. Voltages applied to BLs can enforce a specific switching activity for the output MTJ, which evolves as a function of the resistances (i.e., logic states) of the input MTJs. In other words, voltages applied to BLs can control the switching of the output magnet according to a specific truth table.  A specific voltage range corresponds to each logic gate. This structure can support logic gates of various numbers of inputs.

\ignore{
The type of the logic gate that is implemented is determined by
the number of MTJs in a row that are connected to the LL and the voltages
applied to the BLs. 
Input signals can then be applied via the BLs, which will implement logic
operations.
Specifically,
}

\begin{wrapfigure}{r}{0.3\textwidth}
%
\begin{minipage}{\linewidth}
%\centering
%\captionsetup[subfigure]{justification=centering}
\captionsetup[subfigure]{justification=justified, width=\linewidth}
%   \includegraphics[scale=0.22]{Images/array/3T/cell_memory}
    \includegraphics[width=\linewidth]{Images/array/3T/cell_memory}
    \subcaption{3T1M (memory)}
    \label{fig:cell_memory}
\par\vfill
    \includegraphics[width=\linewidth]{Images/array/3T/cell_logic}
    \subcaption{3T1M (logic)}
    \label{fig:cell_logic}
\end{minipage}
%
\vshrink{.4}
\caption{3T1M cell in memory and logic configuration.}
\label{fig:cell}
\end{wrapfigure}

This design is limited, however, as any logic gate activated  in a row also gets
activated  in {\em all} rows in the array. This is because BLL (which activates
cells to serve as logic gate inputs or outputs) runs through all columns in the array.
%in the fact that
%computation will occur in every row in the array. 
If BLL is set for a
column, MTJs in that column, in all rows, get connected to LL. While such massive row level parallelism may be desirable, it impairs direct adaptation for BNN processing.
%

\vshrink{-.1}
\noindent{\bf Cell \& Array Architecture (3T1M) for \arch:}
To satisfy true PIM semantics, 
%As we are seeking true processing-in-memory semantics, 
we need to perform
computation in only a subset of the rows, while leaving all other rows
unperturbed, which is not the case for~\cite{cram}. 
To achieve this, we can add a 3rd access transistor, as shown in
Fig.\ref{fig:cell_memory} and \ref{fig:cell_logic}. This design preserves the very
same memory interface as a standard STT-MRAM otherwise.
%
%The circuit
%for a cell is shown in Figure \ref{fig:3Tcell}. 
\ignore{
While it is possible to achieve
the same effect without adding a 3rd transistor, it cannot be done without
modifying the circuity dedicated to standard memory operations. The design space
for this problem is rich. 
%However, in this work we show only one representative
%case. 
}
%
%The addition of this 3rd transistor allows MTJs to be activated for logic in a
%subset of the rows and columns within the array. The circuitry for memory
%operation remains unchanged; 
%When no computation takes place, 
%$t_{M}$ is activated by WLM and then BL and BLB are
%used to read and write. 

%The logic functionality is slightly more complex. 
For logic operations, $t_{L}$ from Fig.~\ref{fig:2Tcell} now becomes
%The
%secondary transistor, previously referred to as $t_{L}$ (transistor for logic)
%is relabelled as 
$t_{LC}$ (transistor for logic column). BLL controls $t_{LC}$.
%It is controlled by the
%signal BLL, as before. 
The new signal {\em Wordline for Logic} (WLL) controls the third transistor, $t_{LR}$ (transistor for logic
row).
$t_{LR}$ is in
series with $t_{LC}$, thus, both $t_{LC}$ and $t_{LR}$ must be activated to
connect the MTJ to LL. This enables a row-wise and column-wise specification for
any MTJ to serve as an input or output to a logic gate. BLL and WLL determine
this specification.
%This enables the specification of both the rows and
%the columns for which MTJs are connected to the logic line; the selected MTJs
%are determined by the signals applied to BLL and WLL. 
As all MTJs in a row share
the same LL, still, only one logic operation can be performed in each row at a
time. However, each operation can be performed in any number of the rows
simultaneously. Hence, the array still features row level parallelism. %We provide
%examples of memory and logic operations next.
We next take a closer look into memory and logic semantics.

\vshrink{-.1}
\noindent{\bf Memory \& Logic Semantics (3T1M) for \arch:}
%\noindent{\bf Memory Configuration (3T1M):}
%\subsubsection{CRAM in memory mode}
%To access the array in memory mode, 
Fig.\ref{fig:cell_memory} shows a 3T1M \arch\ cell
activated for memory. 
WLM is set for only one row. This activates
$t_{M}$ and connects MTJs to the BLBs. MTJs can then be read or written via
voltages applied to BL and BLB. In this configuration, the array acts exactly as a
standard STT-MRAM array. For data retention, i.e., if no read or write access is
the case, keeping WLM, WLL, and BLL at logic 0 suffices. 

%\vshrink{-.1}
%\noindent{\bf Logic Configuration (3T1M):}
%\subsubsection{CRAM in logic mode}
Fig.\ref{fig:cell_logic} shows a 3T1M \arch\ cell activated for logic.
WLL is set for all rows in which computation should occur. We follow the same
method as \cite{pinatubo}, and activate rows sequentially. 
%where rows are activated sequentially. 
This
activates $t_{LR}$ for all cells in the row. BLL is set for all columns that
contain inputs and the output. This activates $t_{LC}$ for all cells in the
corresponding columns. Since $t_{LR}$ and $t_{LC}$ are in series, only MTJs that
are in cells with  both activated get connected to LL. 
%This allows the
%specification of inputs and outputs on any specified subset of the rows and
%columns. 
Voltages are applied to the BLs then to specify the type of the logic operation.
%to supply the current for the logic
%operation. 
%A \arch\ cell activated for logic is shown in
%Fig.\ref{fig:cell_logic}. 

\ignore{The demands on our peripheral circuitry are similar to \cite{pinatubo}, though
we use more transistors and do not use sense amplifiers during computation.
Given MTJs are lower power devices, the current draw remains relatively modest
even during highly parallel computation (as detailed in Sect.\ref{sec:setup}).Needs to be moved to a more general location, applying to all designs}



\vshrink{-.1}
%\noindent{\bf Transposed Arrays:}
\noindent{\bf Cell \& Array Architecture (1T1M) for \arch:}
%\subsubsection{Transposed CRAM Arrays}
%\label{sec:transpose}
While the 3T1M design enables selective computing in the \arch\ array (which is
not the case for~\cite{cram}), it incurs the area overhead of an extra
transistor.
%In this section 
We next present an area efficient alternative.
%two solutions which act as alternatives of much lower area
%overhead.
%to the previously described array. 
By taking rotating the logic functionality relative to the
direction of memory operations, we can reduce the number of transistors from
3 to 1, as shown in Fig.\ref{fig:stt}. \blueHL{As the logic functionality is rotated, we refer to this design as \textit{transposed}.}
%
\ignore{
This is the first solution (Fig.\ref{fig:stt}).
\blueHL{The second solution is cell similar to the one found in \cite{masoud2}, which entails }
%A second modification is 
%an addition to this one transistor
%design, where 
the addition of a spin-hall effect (SHE) channel to reduce energy and
latency at the cost of an additional transistor per cell (Fig.\ref{fig:she}). 
}
%
The two MTJs are in adjacent cells in the same column. BL and BLB are replaced
with {\em Bitline Even} (BLE) and {\em Bitline Odd} (BLO). Adjacent MTJs are
connected to different bitlines in this case, BLE and BLO, respectively (and the
connection alternates throughout the column).  {\em Logic Line} (LL) serves both
as the connection between MTJs for logic operations, and also as input for read
and write operations. {\em Wordline} (WL) controls the single access transistor
in each cell, and is used to connect the MTJ to LL.  
%Thus, an MTJ can be
%accessed for a memory operation through LL
%and either RLE or RLO. 


\vshrink{-.1}
\noindent{\bf Memory \& Logic Semantics (1T1M) for \arch:}
%\vshrink{-.1}
%\noindent{\bf Memory Configuration (1T1M):}
When no computation takes place, performing memory operations entails first setting
WL. Specifically, WL gets activated for only one row. This
activates the access transistors and
connects MTJs (in the respective row) to LL. Voltages can then be applied to LL and either
BLE or BLO (depending on the parity of the respective row) for read and write
operations. When compared to the baseline 2T1M design from Fig.\ref{fig:2Tcell},
for memory access,
LL and either of BLE/BLO can be thought of being equivalent to BLB and BL,
respectively. 


%\vshrink{-.1}
%\noindent{\bf Logic Configuration (1T1M):}
For logic on the other hand, WL is set in multiple rows which connects multiple MTJs in a column to LL.
This creates a connection between all activated MTJs that are in the same
column. Voltages are applied to both BLE and BLO in the columns 
where logic gate inputs and outputs reside. 
%in which
%computation should occur.
These voltages determine the type of logic gates performed, in similar nature
to~\cite{cram}.
%provide the current for the logic
%gates.
%
%\redHL{More on mem? Need to mention tri-state buffer for logic?}

This design has the extra restriction that inputs must be in rows that are all
connected to the same type of bitline (i.e., either to BLE or BLO) with the
output connected to the other type: If all inputs are connected to BLE (BLO),
the output must be connected to BLO (BLE). {This is because all input MTJs must
be in parallel with each other and in series with the output MTJ.}
%\redHL{Why?} output with the output connected to the other rowline. 
This may impact data layout, depending on the algorithm being mapped to the
array.  However, \blueHL{the effect is negligible in most operations, including the entire implementation of BNNs. } Due to the reduction to one transistor, the resulting array has
nearly the same density as a standard STT-MRAM array. \blueHL{This is significant as density is a key advantage of STT-MRAM. }



\ignore{
Fig.\ref{fig:she} shows the second solution, which adds
%The second design is shown in Fig.\ref{fig:she}. 
a spin-hall
effect \redHL{\cite{masoud2}} to each MTJ. 
\ignore{
\redHL{Insight: what is this channel good for?}
As a result, all MTJs have three
terminals, instead of two. 
This requires the addition of a second transistor.
One end of the SHE channel is connected directly to the rowline, RLO or RLE,
respectively. The control
signal Bitline Read (BLR) connects the other end of the MTJ to the LL. When BLR is
activated, current travels through the SHE channel and the MTJ. This is used
when reading the MTJ or when the MTJ is the input of a logic gate. The SHE channel
has a significantly lower resistance than the MTJ, thus the state of the MTJ
still dominates the effective resistance.  The third terminal connects the other
end of the SHE channel to the Logic Line (LL). Bitline Write (BLW) activates this
connection and is used when writing to the MTJ or when the MTJ is the output of
a logic operation. When BLR is activated, current only travels through the SHE
channel but can still change the state of the MTJ. \redHL{More structured
discussion on logic and mem semantics? How different would it be to implement a
gate? Rd/Wr semantics? We can tie this to 1T1M discussion, as well.}
}
Passing current through the SHE channel will switch the state of the MTJ. Since the channel has a much lower resistance than the MTJ, it enables faster switching and lower energy consumption. However, it introduces another terminal, making the MTJ a 3-terminal device and necessitates the addition of a second transistor per cell. As a consequence, two signals are required for each row, Wordline Read (WLR) and Wordline Write (WLW). WLR acts nearly identical to WL in that it connects the MTJ to LL. WLW connects the end of the SHE channel to the LL. 

\vshrink{-.1}
\noindent{\bf Memory Configuration (2T1M):}
To perform a read, WLR is set for one row and voltages are applied to the LL and either BLE and BLO. Current travels through the MTJ. To perform a write, WLW, instead of WLR, is set for one row. Current travels through the SHE channel.

\vshrink{-.1}
\noindent{\bf Logic Configuration (2T1M):}
WLR is set in one or more rows that contain input MTJs. WLW is set in one row that contains the output MTJ. Voltages are applied to both BLE and BLO in the columns in which computation should occur. Current travels through the input MTJs and through the SHE channel of the output MTJ.
}
%Saved for eval
\ignore{
This design has multiple
advantages. For all operations, MTJ switching has a lower latency and energy
cost. For logic operations, the effective resistance of the output MTJ is
reduced since current only travels through the SHE channel. This reduced
resistance relative to the input MTJs increases the voltage margins for the
logic operations and, as a consequence, increases reliability. An additional
benefit is that the resistance of the SHE channel is independent of the state,
which removes the need for presetting the value of output MTJs.
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
\begin{table}
\centering
\begin{tabular}{ | c | c | c | c | }
\hline
Operation & WLM & BLL & WLL \\
\hline
Retention & L & L & L \\
\hline
Memory & H & L & L \\
\hline
Logic & L & H & H \\
\hline
\end{tabular}
\caption{Control Signals that are high (H)/low (L) for different operations}
\label{tab:control_signals}
\end{table}
}

\ignore{
\begin{figure}[t!]
\begin{subfigure}[t]{.4\textwidth}
\centering
\includegraphics[scale=0.25]{Images/array/T/STT.png}
\caption{Tranposed CRAM cell}
\label{fig:stt}
\end{subfigure}
\begin{subfigure}[t]{.4\textwidth}
\centering
\includegraphics[scale=0.25]{Images/array/T/SHE}
\caption{Transposed SHE-CRAM cell}
\label{fig:3Tshe}
\end{subfigure}
\caption{Different CRAM cell designs}
\label{fig:SHE}
\end{figure}
}

\ignore{
\begin{figure}[tp]
\begin{subfigure}[t]{.4\columnwidth}
\centering
\includegraphics[scale=0.25]{Images/array/prev/cell.png}
\caption{2T1M cell}
\label{fig:2Tcell}
\end{subfigure}
~~~
\begin{subfigure}[t]{.4\columnwidth}
\centering
\includegraphics[scale=0.2]{Images/array/3T/cell}
\caption{3T1M cell}
\label{fig:3Tcell}
\end{subfigure}
\vshrink{.2}
\caption{Different memory cell architectures.}
\label{fig:cell}
\vshrink{.7}
\end{figure}
}

\ignore{
\begin{figure}[tp]
\begin{subfigure}[t]{.15\textwidth}
\centering
\includegraphics[scale=0.17]{Images/array/3T/cell_memory}
\caption{}
\label{fig:cell_memory}
\end{subfigure}
\begin{subfigure}[t]{.15\textwidth}
\centering
\includegraphics[scale=0.17]{Images/array/3T/cell_logic}
\caption{}
\label{fig:cell_logic}
\end{subfigure}
%\begin{subfigure}[t]{.15\textwidth}
%\centering
%\includegraphics[scale=0.15]{Images/array/gate1}
%\caption{}
%\label{fig:gate1}
%\end{subfigure}
%\begin{subfigure}[t]{.15\textwidth}
%\centering
%\includegraphics[scale=0.15]{Images/array/gate2}
%\caption{}
%\label{fig:gate2}
%\end{subfigure}
\begin{subfigure}[t]{.15\textwidth}
\centering
\includegraphics[scale=0.17]{Images/array/gate3}
\caption{}
\label{fig:gate3}
\end{subfigure}
\vshrink{0.3}
\caption{A \arch\ cell in memory mode (\ref{fig:cell_memory}) and in logic mode
  (\ref{fig:cell_logic}). The number of BLLs set determines the number of inputs.
One row can implement fan-in of one, two, three (\ref{fig:gate3}) or higher.}
%one \ref{fig:gate1}, two \ref{fig:gate2}, three \ref{fig:gate3}, or higher. }
\label{fig:configs}
\vshrink{0.3}
\end{figure}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> mine/data.tex <==



\begin{table*}[p]
\centering
\small
\begin{tabular}{ | c | c | c | c | c | c | c | c | c | c | c | c | c | }
\hline
Network & F & F+N & F+PC & F+PC+N & F+FPC & F+FPC+N & F-T & F-T+N & F-T+PC & F-T+PC+N & F-T+FPC & F-T+FPC+N  \\
\hline
FPBNN Cifar-10  & 5.43e-4 & 6.77e-4 & 3.22e-2 & 3.74e-2 & 2.51e-3 & 2.77e-3 & 3.97e-4 & 5.18e-4 & 4.84e-3 & 4.97e-3 & 7.88e-4 & 8.40e-4   \\
\hline
%FPBNN FC  & 1.30e-4 & 1.45e-4 & 8.46e-3 & 1.02e-2 & 4.26e-4 & 4.91e-4 & 1.85e-4 & 2.28e-4 & 4.63e-4 & 5.05e-4 & 1.98e-4 & 2.41e-4   \\
FPBNN FC  & 1.30e-4 & 1.45e-4 & 8.46e-3 & 1.02e-2 & 4.26e-4 & 4.91e-4 & 5.97e-5 & 7.42e-5 & 4.63e-4 & 5.05e-4 & 1.98e-4 & 2.41e-4   \\
\hline
FINN Cifar-10  & 2.77e-4 & 3.32e-4 & 1.56e-2 & 1.85e-2 & 1.17e-3 & 1.30e-3 & 1.85e-4 & 2.58e-4 & 9.45e-4 & 1.01e-3 & 3.35e-4 & 3.58e-4   \\
\hline
FINN FC  & 3.05e-5 & 3.47e-5 & 2.48e-3 & 2.98e-3 & 1.07e-4 & 1.20e-4 & 1.57e-5 & 1.78e-5 & 2.11e-4 & 2.24e-4 & 6.06e-5 & 6.31e-5   \\
\hline
\end{tabular}
\caption{ Latencies (s) for each Future network for different configurations. F=Future, M=Modern, (P)=Peripheral Circuitry, (FP)=Future Peripheral Circuitry, (N)=NAND and NOT only) }
\label{ tab:refdata_lf }
\end{table*}

\begin{table*}[p]
\centering
\small
\begin{tabular}{ | c | c | c | c | c | c | c | c | c | c | c | c | c | }
\hline
Network & F & F+N & F+PC & F+PC+N & F+FPC & F+FPC+N & F-T & F-T+N & F-T+PC & F-T+PC+N & F-T+FPC & F-T+FPC+N \\
\hline
FPBNN Cifar-10  & 1.87e-5 & 2.76e-5 & 2.12e-3 & 2.47e-3 & 1.89e-5 & 2.78e-5 & 1.87e-5 & 2.76e-5 & 3.07e-4 & 3.16e-4 & 1.88e-5 & 2.77e-5   \\
\hline
%FPBNN FC  & 6.23e-7 & 9.25e-7 & 5.51e-4 & 6.68e-4 & 6.34e-7 & 9.29e-7 & 6.08e-7 & 9.02e-7 & 1.93e-5 & 1.96e-5 & 6.09e-7 & 9.03e-7   \\
FPBNN FC  & 6.23e-7 & 9.25e-7 & 5.51e-4 & 6.68e-4 & 6.34e-7 & 9.29e-7 & 6.23e-7 & 9.20e-7 & 1.93e-5 & 1.96e-5 & 6.09e-7 & 9.03e-7   \\
\hline
FINN Cifar-10  & 5.42e-6 & 7.95e-6 & 1.02e-3 & 1.21e-3 & 6.57e-6 & 8.08e-6 & 5.42e-6 & 7.95e-6 & 4.83e-5 & 5.12e-5 & 6.53e-6 & 8.02e-6   \\
\hline
FINN FC  & 8.51e-8 & 1.28e-7 & 1.61e-4 & 1.95e-4 & 9.18e-8 & 1.32e-7 & 8.51e-8 & 1.28e-7 & 1.07e-5 & 1.08e-5 & 9.00e-8 & 1.29e-7   \\
\hline
\end{tabular}
\caption{ Energies (J) for each Future network for different configurations. F=Future, M=Modern, (P)=Peripheral Circuitry, (FP)=Future Peripheral Circuitry, (N)=NAND and NOT only) }
\label{ tag:refdata_ef }
\end{table*}

\begin{table*}[p]
\centering
\small
\begin{tabular}{ | c | c | c | c | c | c | c | c | c | }
\hline
Network & M & M+N & M+PC & M+PC+N & M-T & M-T+N & M-T+PC & M-T+PC+N  \\
\hline
FPBNN Cifar-10  & 1.63e-03 & 2.03e-03 & 3.44e-02 & 3.98e-02 & 1.19e-03 & 1.56e-03 & 5.98e-03 & 6.35e-03   \\
\hline
FPBNN FC  & 3.90e-04 & 4.35e-04 & 9.06e-03 & 1.09e-02 & 5.56e-04 & 6.84e-04 & 8.33e-04 & 9.61e-04   \\
\hline
FINN Cifar-10  & 8.31e-04 & 9.97e-04 & 1.68e-02 & 1.98e-02 & 5.54e-04 & 7.73e-04 & 1.58e-03 & 1.78e-03   \\
\hline
FINN FC  & 9.13e-05 & 1.04e-04 & 2.65e-03 & 3.18e-03 & 4.71e-05 & 5.35e-05 & 3.18e-04 & 3.54e-04   \\
\hline
\end{tabular}
\caption{ Latencies (s) for each Modern network for different configurations. F=Future, M=Modern, (P)=Peripheral Circuitry, (FP)=Future Peripheral Circuitry, (N)=NAND and NOT only) }
\label{ tab:refdata_lm }
\end{table*}

\begin{table*}[p]
\centering
\small
\begin{tabular}{ | c | c | c | c | c | c | c | c | c | }
\hline
Network & M & M+N & M+PC & M+PC+N & M-T & M-T+N & M-T+PC & M-T+PC+N  \\
\hline
FPBNN Cifar-10  & 1.20e-03 & 1.64e-03 & 3.30e-03 & 4.08e-03 & 1.20e-03 & 1.64e-03 & 1.49e-03 & 1.92e-03   \\
\hline
FPBNN FC  & 4.00e-05 & 5.49e-05 & 5.90e-04 & 7.21e-04 & 3.92e-05 & 5.37e-05 & 5.79e-05 & 7.24e-05   \\
\hline
FINN Cifar-10  & 3.49e-04 & 4.72e-04 & 1.40e-03 & 1.73e-03 & 3.49e-04 & 4.72e-04 & 4.29e-04 & 5.70e-04   \\
\hline
FINN FC  & 5.47e-06 & 7.58e-06 & 1.67e-04 & 2.02e-04 & 5.47e-06 & 7.58e-06 & 1.61e-05 & 1.81e-05   \\
\hline
\end{tabular}
\caption{ Energies (J) for each Modern network for different configurations. F=Future, M=Modern, (P)=Peripheral Circuitry, (FP)=Future Peripheral Circuitry, (N)=NAND and NOT only) }
\label{ tag:refdata_em }
\end{table*}


\begin{table*}[p]
\centering
\small
\begin{tabular}{ | c | c | c | c | c | c | c | }
\hline
Network & F-T & F-T+N & F-T+PC & F-T+PC+N & F-T+FPC & F-T+FPC+N  \\
\hline
FPBNN Cifar-10  & 5.23e-6 & 8.01e-6 & 2.94e-4 & 2.96e-4 & 5.27e-6 & 8.02e-6   \\
\hline
FPBNN FC  & 1.72e-7 & 2.63e-7 & 1.89e-5 & 1.90e-5 & 1.72e-7 & 2.63e-7   \\
\hline
FINN Cifar-10  & 1.53e-6 & 2.31e-6 & 4.40e-5 & 4.49e-5 & 1.84e-6 & 2.33e-6   \\
\hline
FINN FC  & 2.39e-8 & 3.72e-8 & 1.07e-5 & 1.07e-5 & 2.46e-8 & 3.66e-8   \\
\hline
\end{tabular}
\caption{ Energies (J) for each Future SHE network for different configurations. F=Future, M=Modern, (P)=Peripheral Circuitry, (FP)=Future Peripheral Circuitry, (N)=NAND and NOT only) }
\label{ tag:refdata_efs }
\end{table*}

\begin{table*}[p]
\centering
\small
\begin{tabular}{ | c | c | c | c | c | }
\hline
Network & M-T & M-T+N & M-T+PC & M-T+PC+N  \\
\hline
FPBNN Cifar-10  & 3.76e-4 & 5.33e-4 & 6.64e-4 & 8.19e-4   \\
\hline
FPBNN FC  & 1.23e-5 & 1.75e-5 & 3.10e-5 & 3.62e-5   \\
\hline
FINN Cifar-10  & 1.10e-4 & 1.53e-4 & 1.64e-4 & 2.14e-4   \\
\hline
FINN FC  & 1.71e-6 & 2.46e-6 & 1.24e-5 & 1.31e-5   \\
\hline
\end{tabular}
\caption{ Energies (J) for each Modern SHE network for different configurations. F=Future, M=Modern, (P)=Peripheral Circuitry, (FP)=Future Peripheral Circuitry, (N)=NAND and NOT only) }
\label{ tag:refdata_ems }
\end{table*}

==> mine/data_notUsed.tex <==
\section{Data}
Data Tables for reference
\begin{table}
\begin{tabular}{ | c | c | c | c | c | c | c | c | }
\hline
 Network & FPGA & F & F (FPC+N) & F-T & F-T (FPC+N) & M \\ 
 \hline
FPBNN Cifar-10 &  1.30e-04  & 5.43e-04 & 1.30e-03 & 3.97e-04 & 8.40e-04 & 1.63e-03 \\
\hline
FPBNN FC &  3.39e-06  & 1.30e-04 & 2.48e-04 & 2.27e-05 & 2.16e-03 & 3.90e-04 \\
\hline
FINN Cifar-10 &  2.83e-04  & 2.77e-04 & 5.52e-04 & 1.85e-04 & 3.58e-04 & 8.31e-04 \\
\hline
FINN FC &  2.44e-06  & 3.05e-05 & 6.72e-05 & 1.57e-05 & 6.31e-05 & 9.13e-05 \\
\hline
\end{tabular}
\caption{ Latencies (s) for each network for different configurations. F=Future, M=Modern, (P)=Peripheral Circuitry, (FP)=Future Peripheral Circuitry, (N)=NAND and NOT only) }
\label{ tab:totals_l }
\end{table}

\begin{table}
\begin{tabular}{ | c | c | c | c | c | c | c | c | }
\hline
 Network & FPGA & F & F (FPC+N) & F-T & F-T (FPC+N) & M \\ 
 \hline
FPBNN Cifar-10 &  3.41e-03  & 1.99e-06 & 3.06e-06 & 1.99e-06 & 3.06e-06 & 4.64e-03 \\
\hline
FPBNN FC &  8.88e-05  & 6.65e-08 & 1.01e-07 & 7.05e-08 & 1.32e-07 & 1.54e-04 \\
\hline
FINN Cifar-10 &  1.02e-03  & 5.79e-07 & 8.86e-07 & 5.79e-07 & 8.85e-07 & 1.34e-03 \\
\hline
FINN FC &  2.15e-05  & 9.10e-09 & 1.43e-08 & 9.10e-09 & 1.44e-08 & 2.12e-05 \\
\hline
\end{tabular}
\caption{ Energies (J) for each network for different configurations. F=Future, M=Modern, (P)=Peripheral Circuitry, (FP)=Future Peripheral Circuitry, (N)=NAND and NOT only) }
\label{ tab:totals_e }
\end{table}



\begin{table}
\begin{tabular}{ | c | c | c | c | c | c | c | c | }
\hline
 Network & FPGA & F & F (FPC+N) & F-T & F-T (FPC+N) & M \\ 
 \hline
FPBNN Cifar-10 &  1.30e-04  & 5.43e-04 & 1.30e-03 & 3.97e-04 & 8.40e-04 & 1.63e-03 \\
\hline
FPBNN FC &  3.39e-06  & 1.30e-04 & 2.48e-04 & 2.27e-05 & 2.16e-03 & 3.90e-04 \\
\hline
FINN Cifar-10 &  2.83e-04  & 2.77e-04 & 5.52e-04 & 1.85e-04 & 3.58e-04 & 8.31e-04 \\
\hline
FINN FC &  2.44e-06  & 3.05e-05 & 6.72e-05 & 1.57e-05 & 6.31e-05 & 9.13e-05 \\
\hline
\end{tabular}
\caption{ Latencies (s) for each network for different configurations. F=Future, M=Modern, (P)=Peripheral Circuitry, (FP)=Future Peripheral Circuitry, (N)=NAND and NOT only) }
\label{ tab:totals_sl }
\end{table}

\begin{table}
\begin{tabular}{ | c | c | c | c | c | c | c | c | }
\hline
 Network & FPGA & F & F (FPC+N) & F-T & F-T (FPC+N) & M \\ 
 \hline
FPBNN Cifar-10 &  3.41e-03  & 1.99e-06 & 3.06e-06 & 1.72e-06 & 2.65e-06 & 4.64e-03 \\
\hline
FPBNN FC &  8.88e-05  & 6.65e-08 & 1.01e-07 & 6.12e-08 & 1.19e-07 & 1.54e-04 \\
\hline
FINN Cifar-10 &  1.02e-03  & 5.79e-07 & 8.86e-07 & 4.98e-07 & 7.65e-07 & 1.34e-03 \\
\hline
FINN FC &  2.15e-05  & 9.10e-09 & 1.43e-08 & 7.84e-09 & 1.26e-08 & 2.12e-05 \\
\hline
\end{tabular}
\caption{ Energies (J) for each network for different configurations. F=Future, M=Modern, (P)=Peripheral Circuitry, (FP)=Future Peripheral Circuitry, (N)=NAND and NOT only) }
\label{ tab:totals_se }
\end{table}



==> mine/datalayout.tex <==
\subsubsection{2-dimensional Data Layout Optimization}
\label{sec:datalayout}
CRAM is a 2-dimensional substrate. However, data parallelism exists only in one dimension. Operations can be performed in each row simultaneously but multiple operations in the same row must be performed sequentially. Parallelism can be increased by using more rows, but this introduces a requirement to perform intermediate reads and writes between rows. This creates a trade-off space between row parallelism and communication cost. Splitting a single computation into more rows decreases computation time but has a higher communication overhead between rows. This is because the intermediate results, which must be placed in a single row to compute the final result, will be spread across a greater number of rows. The simplest representative example of this trade-off is a NAND dot product.

A NAND dot product is a bit-wise NAND of two vectors, followed by a summation of the resulting bits. NAND gates can be completed in a single cycle in CRAM. Binary full adder trees are used to perform summation. In a two-dimensional layout, a dot product will consist of four steps:
\begin{enumerate}
\item bitwise NAND
\item simultaneous summation of bits on each row
\item copy of sums to a single row 
\item summation of intermediate sums to produce the final result
\end{enumerate}
The optimal layout depends on the complexities of each of the steps. The lengths of steps 2 and 4 depend on the chosen summation algorithm and the gate types used. Step 3 depends on the peripheral circuitry overheads, which vary considerably depending on the specific CRAM configuration. Each design can have a unique optimal configuration but certain trends hold for all designs. Larger numbers of outputs and increased peripheral circuitry overhead favor using fewer numbers of rows (fewer rows are used for the computation of each output). This is because the number of data transfers required scale with the number of outputs being computed. In the example, only one final output is produced. However, typically many outputs are computed simultaneously, and each will require the same amount of transfers. The cost of peripheral circuitry will make each of these transfers take longer and consume more energy. Larger inputs favor using larger numbers of rows. If there are a large number of inputs for every output, the computation can be sufficiently long to benefit from increased parallelism, even with the addition costly communication cost. 

Fully-Connected and convolutional layers of binary neural networks in CRAM are similar to dot products. The only difference is that XNOR replaces NAND and there are additional batch normalization and comparison computations. Convolutional layers typically have fewer input neurons and more output neurons than fully-connected layers. Thus, output neurons of convolution layers typically are computed in only a single row, whereas output neurons of fully-connected layers typically use multiple rows. 



==> mine/feFigTMP.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
\begin{wrapfigure}{l}{0.3\textwidth}

%
\begin{minipage}{\linewidth}
\centering
%\captionsetup[subfigure]{justification=centering}
\captionsetup[subfigure]{justification=justified, width=\linewidth}
%   \includegraphics[scale=0.22]{Images/array/3T/cell_memory}
    \includegraphics[width=\linewidth]{Images/array/prev/cell.png}
    \subcaption{2T1M~\cite{cram}}
\label{fig:2Tcell}
\par\vfill
    \includegraphics[width=.85\linewidth]{Images/array/T/STT.png}
    \subcaption{1T1M}
\label{fig:stt}
\end{minipage}
%
\vshrink{.4}
%\caption{Default 2T1M vs. 1T1M cell.}
\caption{Cell architecture.}
\label{fig:basiccell}
\vshrink{.3}
\end{wrapfigure}
}

\ignore{
\begin{wrapfigure}{r}{0.3\textwidth}
%
\begin{minipage}{\linewidth}
%\centering
%\captionsetup[subfigure]{justification=centering}
\captionsetup[subfigure]{justification=justified, width=\linewidth}
%   \includegraphics[scale=0.22]{Images/array/3T/cell_memory}
    \includegraphics[width=\linewidth]{Images/array/3T/cell_memory}
    \subcaption{3T1M (memory)}
    \label{fig:cell_memory}
\par\vfill
    \includegraphics[width=\linewidth]{Images/array/3T/cell_logic}
    \subcaption{3T1M (logic)}
    \label{fig:cell_logic}
\end{minipage}
%
\vshrink{.4}
\caption{3T1M cell in memory and logic configuration.}
\label{fig:cell}
\end{wrapfigure}
}

\ignore{
\begin{figure*}[tp]
\begin{subfigure}[t]{.35\columnwidth}
\centering
\includegraphics[scale=0.22]{Images/array/prev/cell.png}
\caption{2T1M }
\label{fig:2Tcell}
\end{subfigure}
~~~
\begin{subfigure}[t]{.3\columnwidth}
\centering
\includegraphics[scale=0.22]{Images/array/3T/cell_memory}
\caption{3T1M (memory)}
\label{fig:cell_memory}
\end{subfigure}
~~
\begin{subfigure}[t]{.3\columnwidth}
\centering
\includegraphics[scale=0.22]{Images/array/3T/cell_logic}
\caption{3T1M (logic)}
\label{fig:cell_logic}
\end{subfigure}
%\begin{subfigure}[t]{.4\columnwidth}
%\centering
%\includegraphics[scale=0.2]{Images/array/3T/cell}
%\caption{3T1M cell}
%\label{fig:3Tcell}
%\end{subfigure}
\begin{subfigure}[t]{.45\columnwidth}
\centering
\includegraphics[scale=0.23]{Images/array/T/STT.png}
\caption{Tranposed 1T1M}
\label{fig:stt}
\end{subfigure}
\begin{subfigure}[t]{.45\columnwidth}
\centering
\includegraphics[scale=0.2]{Images/array/T/SHE}
\caption{Transposed SHE}
\label{fig:she}
\end{subfigure}

\caption{Different cell architectures.}
\label{fig:cell}

\end{figure*}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> mine/knet.tex <==
\subsection{K-NET}
\label{sec:knet}
\blueHL{woops, this is duplicate}We introduce a customized binarized neural network, K-NET, which finds if two strings of genomic information match or not. [POTENTIAL CITATION HERE.] It is used as part of a larger genetic algorithm and it achieves an accuracy of 93.4\%, on average. To the best of our knowledge, this is the first use of a binarized neural network for similarity matching in genetic applications. The core operations are the same as other binary networks, however convolution can occur in different dimensions for different layers. Additionally, the layer sizes are non-uniform, which are listed in Table \ref{tab:knet}. As this network is the first of its kind, there is no direct baseline for comparison. Given \cite{FPBNN} is an FPGA specifically tailored for binary neural networks, which significantly outperforms CPU and GPU implementations, we believe it is the best known substrate to implement K-NET. Using reported layer sizes and latencies from \cite{FPBNN}, we extract a latency and energy model for the performance of an arbitrarily sized network on the FPGA. Using the same approach as for the previously described networks, we schedule K-NET on \arch\ and report the simulated latency and energy consumption. The results are listed in Table \ref{tab:knetpl}. Consistent with previous findings, the FPGA is faster but \arch\ is much more energy efficient.  

\begin{table*}[t]
\begin{tabular}{  c | c | c | c | c | c | c  }
%\hline
Layer & Type & Input & Num Filters & Filter Size & Pool Size & Output  \\
\hline
1 & Conv & 4x100x1 & 64 & 4x3 & 1x5 & 1x20x64 \\
%\hline
2 & Conv & 1x20x64 & 32 & 1x5x64 & 1x2 & 1x10x32 \\
%\hline 
3 & Conv & 1x10x32 & 20 & 1x4x32 & 1x2 & 1x5x20 \\
%\hline 
4 & FC & 100 & - & - & - & 40 (10-bit) \\
%\hline
\end{tabular}
\caption{K-NET Layers}
\label{tab:knet}
\end{table*}

\begin{table}
    \centering
    \begin{tabular}{c|c|c|c}
         & FP-BNN \cite{FPBNN} & \arch\ F-T & \arch\ F-T (FPC+N)\\
        \hline
        Latency (s) & 9.95e-8 & 1.73e-5 & 2.61e-5 \\
        Energy (J) & 2.37e-7 & 6.93e-9 & 9.81e-9
    \end{tabular}
    \caption{Latency and Energy for K-NET on different platforms}
    \label{tab:knetpl}
\end{table}

==> mine/motiv.tex <==
\noindent While individual operations are slower in \arch\ than CMOS logic, \arch\ can exploit
a high degree of parallelism, which allows it to achieve considerable
throughput. To find the upper bound on \arch 's performance, we ignore the
overheads due to peripheral circuitry and determine the rate at which it can
perform bit-wise operations. To compare this to other memory platforms, we take
data from \cite{ambit}, which is an in-memory bit-wise platform in DRAM. They
compare their bit-wise throughput on 32MB vectors to an Intel Skylake CPU
\cite{skylake}, an NVIDIA GeForce GTX 745 GPU \cite{gtx}, and the logic layer of
an HMC 2.0 \cite{hmc}. These throughputs, along with throughputs for \arch, are
shown in Figure \ref{fig:gops}. We assume a similar memory size as Ambit. They
report using 8 banks of a standard DRAM module. We assume one 128 MB bank, which
has a configuration taken from NVSIM \cite{nvsim}. All bit-wise operations in
\arch\ take the same time. The throughputs for XOR/XNOR are lower as XOR/XNOR
cannot be performed directly and must be implemented in multiple steps. Another
major advantage of \arch is that it is highly energy efficient. This makes \arch\
appropriate not only for high performance accelerators, but also for mobile
applications. The potential energy efficiency is shown in Figure \ref{fig:opsw},
where operations per watt per second are reported. In addition to being highly
energy efficient during computation, \arch\ is non-volatile, which enables it to
have a near zero standby power. We also compare \arch s throughput with Pinatubo
\cite{pinatubo}, which is a non-volatile in-memory computing substrate which
performs computation using the sense amplifiers. For bit-wise OR operations,
they report a maximal throughput of 8,000 GBps, which is performed on vectors of
length $2^{19}$ or larger. Using the same input, \arch\ can achieve 8,192 GBps.
Thus, \arch\ is a substrate that is capable of high computational throughput
without the use of any peripheral logic circuits. It is also highly energy
efficient, has zero standby power, and can be used as non-volatile memory. 

\begin{figure*}[t]
\begin{subfigure}{.4\textwidth}
\centering
\includegraphics[scale=0.35]{gops}
\caption{Bitwise GOps/s on different platforms. Taken from \cite{ambit}}
\label{fig:gops}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
\centering
\includegraphics[scale=0.35]{opsw}
\caption{Bitwise Ops/s/w on different platforms. Taken from \cite{ambit}}
\label{fig:opsw}
\end{subfigure}
\caption{Bitwise throughput and energy efficiency comparisons of \arch\ to other platforms}
\label{fig:bitwisecomparison}
\end{figure*}























==> mine/response.tex <==
\section*{Response to Reviewers}
We thank the editors and the reviewers for very useful and constructive feedback.
%
Following this feedback, we have modified our simulations to provide more intuitive results. Specifically, we have made the following changes:
\begin{enumerate}
    \item We exclusively use robust NOT, NAND, and COPY gates, as opposed to using both this set and a larger (but less reliable) set of gates.
    \item We no longer report results for the combination of modern peripheral circuitry with future MTJ devices. Rather we only use future peripheral circuitry estimates with future MTJ devices.
    \item We use smaller arrays, which significantly increases parallelism and performance at the cost of energy efficiency. This fits a design target of high performance accelerator, which is more appropriate given the amount of memory we are using.
    \item We compare different sizes of arrays rather than assuming a single size.
    \item We only consider one cell design in the evaluation as using different cell designs only corresponds to a slightly modified data layout. Additionally, we believe the 1T design to be more practical than the 3T.
    \item We report memory usage in bytes 
    %as our x-axis, 
    rather than number of arrays.
%    \item We discovered an error in both our BioNet simulations and model for BioNet on FPGA. This resulted in us loosing confidence in the FPGA model and we have abandoned it.
\end{enumerate}
As a consequence of the above changes, the latency of our design is now competitive with our baselines. As a direct consequence, the throughput of our pipelined designs are considerably higher. We still maintain a better energy efficiency and low power.

Finally, we also changed our name to avoid a naming conflict with the recently published paper {\em SimBNN: A Similarity-Aware Binarized Neural Network Acceleration Framework}. \\


\noindent \textbf{Reviewer-2:}\\

\noindent \textbf{R2.1.} \textit{The authors should look at how threshold currents for access transistors (Vth) influence their output voltages. The authors do not talk about what the operational voltages are. All the word-lines and bit-lines cannot be operated at the same voltage (at least I think they can't, I may be wrong). This is because there will be voltage drops across the access transistors, especially for the 3T designs.}\\

\noindent We added a discussion of impact of access transistors to section \ref{sec:systemconfig}. We expanded upon that with a brief discussion of process variation. In short, we can set the bit lines to the appropriate voltages since the number of transistors in series with the MTJs remains constant, and the number of which is determined at design time. This allows us to account for their presence by modifying the voltage levels that would be applied for each operation.\\

 \noindent \textbf{R2.2.} \textit{Based on point 1 above, x-point memory architectures suffer from huge leakage currents and voltages that cause neighboring cells to flip incorrectly. The authors should analyze this phenomenon and describe it with some numbers. This may cause a loss in accuracy for BNNs. This may not be a problem in 3T architectures.}\\
%We added some discussion about our relation to cross bar architectures in section \ref{sec:cram}. 

\noindent {The similarity of \arch\ to MRAM gives it some advantages over other PIM technologies. Notably, the high ON/OFF ratio of the CMOS access transistors prevents large leakage currents and the circuitry of individual cells are well isolated. Hence, we assume that we can perform operations in the array free of error. This is in contrast to crossbar type architectures, such as Intel's x-point, where corruption of neighboring cells is possible due to voltage spikes. }
%In short, our architecture is more similar to an STT-MRAM array, and we benefit from the use of high ON/OFF current access CMOS transistors. As a result, we are assuming we can operate free of error and that the output of the program in the array is correct. \\

\newpage
\noindent \textbf{Reviewer-3:}\\
 
\noindent \textbf{R3.1.} \textit{Three missing references, two qualitative and one quantitative comparison...}\\

\noindent We have included references to Neurocube [ISCA-2016] and Tetris [ASPLOS-2017] in our related work section and gave a brief comparison to our work. 

We have included a reference to {\em Accelerating binarized neural networks: Comparison of FPGA, CPU, GPU, and ASIC} by Nurvitadhi et. al. in our related work section. We realize the reviewer asked for a quantitative comparison to this work. Unfortunately, we were unable to do this due to the manner in which results are reported in the paper. They report all results relative to a CPU baseline, and the metrics of interest to us (throughput, latency, energy) are not reported for their baseline. Additionally, they appear to only be evaluating performance for a single layer of each network, whereas our baselines are evaluating the entire network. As a result, we do not believe a direct comparison to our work is possible.

However, we believe this not to be too unfortunate as our baselines, FINN [Umuroglu et. al. 2017] and FP-BNN [Liang et al. 2018], were published after and appear to claim significantly higher performance. For example, for a fully connected layer of AlexNet, Nurvitadhi et. al. report less than a 10$\times$ speedup relative to a binarized CPU (Intel Xeon E5-2966v3) implementation and approximately the same performance as a binarized GPU (Titan X) implementation. On the same layer configuration, Liang et al. report more than 700$\times$ improvement over CPU (Intel E5-2640) and 70$\times$ improvement over GPU (Tesla K40). Admittedly, the CPU/GPU used by Nurvitadhi are higher performance (but comparable) to those used by Liang. However, we believe the significant difference in reported improvement more than compensates for this difference.


%Nurvitadhi et. al. compare relative to an Intel Xeon E5-2966v3 processor running non-binarized models, and their highest performance binzarized configurations achieve slightly greater than a 100x improvement. Our baseline, Liang et. al. compare to an Intel E5-2640 (a lower performance, but comparable CPU) running optimized and binarized models, and report more than a 300x speedup with their FPGA design.

==> mine/setup.tex <==
\subsubsection{The Magnetic Tunnel Junction}
The magnetic tunnel junction (MTJ) is the building block of the CRAM array. MTJs
are a resistive memory devices.  Each MTJ has two magnetic layers, a fixed layer
and a free layer. The polarity of the free layer can change but the fixed
cannot. When the two layers are aligned, the MTJ is in the parallel (P) state,
which considered to be logical 0. If the magnetic layers are not aligned, the
MTJ is in the anti-parallel (AP) state, which is considered to be logical 1. The
MTJ has a much higher resistance in the AP state than it does the P state. That
state can be changed by passing current through the device. The direction of the
current determines the state. When electrons travel from the fixed layer to the
free layer, the MTJ is switched to the P state. The reverse direction sets the
MTJ to the AP state. The threshold current, $I_{C}$, is the current at which the
MTJ has a 50\% chance of switching within the switching time $T_{switch}$. By
setting the write current to 1.5*$I_{C}$, switching will occur with a
probability of error less than $10^{-5} $. The MTJ parameters $I_{C}$ and
$T_{switch}$ are determined by the fabrication process of the device.

\subsubsection{Array Structure}
The CRAM arrays assumed in this work have a capacity of 128MB. We use a
configuration suggested by NVSIM \cite{nvsim} for an STT-MRAM array. Each array
is a single bank which consists of 256 Mats. Mats are organized into 32 rows and
8 columns. Each mat contains 2x2=4 subarrays which are each of size 1024x1024. A
total of 32*2*1024=65536 rows can be activated for computation simultaneously.
The estimates for energy and latency due to peripheral circuitry are also taken
from NVSIM. While the method by which CRAM performs computation is different,
the array structure is similar to that found in~\cite{pinatubo}.


